Determining the unitarity triangle angle $\gamma$ with a four-body amplitude analysis of $\rm B^\pm \to (K^+K^-\pi^+\pi^-)_D K^\pm$ decays

We explain how a four-body amplitude analysis of the $\rm D$ decay products in the mode $\rm B^\pm \to (K^+K^-\pi^+\pi^-)_D K^\pm$ is sensitive to the unitarity triangle angle $\gamma$. We present results from simulation studies which show that a precision on $\gamma$ of $15^\circ$ is achievable with 1000 events and assuming a value of 0.10 for the parameter $r_B$.

==> defs.tex <==
\RequirePackage{xspace}
% A fresh set of definitions for a new year...
%% handy guy to define things for use in or out of math mode
%\def\ifmath#1{\relax\ifmmode #1\else $#1$\fi}%

%\renewcommand {\rm} {\mathrm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  Define private commands here %%%%%%%%%%
% charge specific
\def\BmtoDK      {\ensuremath{\rm B^- \to D^0 K^-}\xspace}
\def\BmtoDbK     {\ensuremath{\rm B^- \to \bar{D}^0 K^-} \xspace}
\def\BmtoD2k2pK  {\ensuremath{\rm B^- \to (K^+K^-\pi^+\pi^-)_D K^-}\xspace}
\def\BptoDK      {\ensuremath{\rm B^+ \to D^0 K^+}\xspace}
\def\BptoDbK     {\ensuremath{\rm B^+ \to \bar{D}^0 K^+} \xspace}
\def\BptoD2k2pK   {\ensuremath{\rm B^+ \to (K^+K^-\pi^+\pi^-)_D \, K^+}\xspace}
\def\Dto2k2p     {\ensuremath{\rm D^0 \to K^+K^-\pi^+\pi^-}\xspace}
\def\Dbto2k2p     {\ensuremath{\rm \bar{D}^0 \to K^+K^-\pi^+\pi^-}\xspace}
% both
\def\BbtoD2k2pK   {\ensuremath{\rm B^\pm \to (K^+K^-\pi^+\pi^-)_D\, K^\pm}\xspace}
\def\BbtoDKfull   {\ensuremath{\rm B^\pm \to D K^\pm \to (K^+K^-\pi^+\pi^-)_D \, K^\pm}\xspace}
% generic
\def\BgtoDKfull   {\ensuremath{\rm B \to D K \to (K^+K^-\pi^+\pi^-)_D \, K}\xspace}
\def\BgtoDK       {\ensuremath{\rm B^\pm \to D K^\pm}\xspace}
\def\BgtoD2k2pK   {\ensuremath{\rm B \to (K^+K^-\pi^+\pi^-)_D \, K}\xspace}
\def\Dgto2k2p     {\ensuremath{\rm D \to K^+K^-\pi^+\pi^-}\xspace}
\newcommand{\prt}[1]{\ensuremath{\mathrm{#1}}}
%%%


